MixTrain: Scalable Training of Verifiably Robust Neural Networks

Making neural networks robust against adversarial inputs has resulted in an arms race between new defenses and attacks. The most promising defenses, adversarially robust training and verifiably robust training, have limitations that restrict their practical applications. The adversarially robust training only makes the networks robust against a subclass of attackers and we reveal such weaknesses by developing a new attack based on interval gradients. By contrast, verifiably robust training provides protection against any L-p norm-bounded attacker but incurs orders of magnitude more computational and memory overhead than adversarially robust training. We propose two novel techniques, stochastic robust approximation and dynamic mixed training, to drastically improve the efficiency of verifiably robust training without sacrificing verified robustness. We leverage two critical insights: (1) instead of over the entire training set, sound over-approximations over randomly subsampled training data points are sufficient for efficiently guiding the robust training process; and (2) We observe that the test accuracy and verifiable robustness often conflict after certain training epochs. Therefore, we use a dynamic loss function to adaptively balance them for each epoch. We designed and implemented our techniques as part of MixTrain and evaluated it on six networks trained on three popular datasets including MNIST, CIFAR, and ImageNet-200. Our evaluations show that MixTrain can achieve up to $95.2\%$ verified robust accuracy against $L_\infty$ norm-bounded attackers while taking $15$ and $3$ times less training time than state-of-the-art verifiably robust training and adversarially robust training schemes, respectively. Furthermore, MixTrain easily scales to larger networks like the one trained on ImageNet-200, significantly outperforming the existing verifiably robust training methods.

==> discussion.tex <==
\section{Discussion}




==> implementation.tex <==
\section{Implementation}
\label{sec:implementation}

\noindent\textbf{Setup.} We implement \sys in \texttt{C} and leverage \texttt{OpenBLAS}\footnote{http://www.openblas.net/} to enable efficient matrix multiplications. 
We evaluate \sys on a Linux server running Ubuntu 16.04 with 16 CPU cores and 256GB memory.

\noindent\textbf{Parallelization.} One unique advantage of \sys over other security property checking systems like Reluplex is that the interval arithmetic in the setting of verifying DNNs is highly parallelizable by nature.
During the process of \iir, newly created input ranges can be checked independently. This feature allows us to create as many threads as possible, each taking care of a specific input range, to gain significant speedup by distributing different input ranges to different workers.

However, there are two key challenges that required solving to fully leverage the benefits of parallelization. First, as shown in Section~\ref{subsec:iir}, the bisection tree is often not balanced leading to substantially different running times for different threads. We found that often several laggard threads slow down the computation, i.e., most of the available workers stay idle while only a few workers keep on refining the intervals. Second, as it is hard to predict the depth of the bisection tree for any sub-interval in advance, starting a new thread for each sub-interval may result in high scheduling overhead. To solve these two problems, we develop a dynamic thread rebalancing algorithm that can identify the potentially deeper parts of the bisection tree and efficiently redistribute those parts among other workers.
 
%Specifically, we keep a sliding window of latest ten depths for each thread to track its current average depth and estimate the depths of following subtrees. 
%Based on such estimated average depth, child threads can be created by \sys to help the slowest thread while minimizing the cost of creating new threads.

\noindent\textbf{Outward rounding.} The large number of floating matrix multiplications in a DNN can potentially lead to severe precision drops after rounding~\cite{goldberg1991every}. 
For example, assume that the output of one neuron is [0.00000001, 0.00000002].
If the floating-point precision is $e-7$, then it is automatically rounded up to [0.0,0.0]. 
After one layer propagation with a weight parameter of 1000, the correct output should be [0.00001, 0.00002]. However, after rounding, the output will incorrectly become [0.0, 0.0]. As the interval propagates through the neural network, more errors will accumulate and significantly affect the output precision. In fact, our tests show that some adversarial examples reported by Reluplex~\cite{katz2017reluplex} are false positives due to such rounding problem.

To avoid such issues, we adopt outward rounding in \sys. 
In particular, for every newly calculated interval or symbolic interval, we always round the bounds outward to ensure the computed output range is always a sound overestimation of the true output range. We implement outward rounding with 32-bit floats. We find that this precision is enough for verifying properties of ACAS Xu models, though it can easily be extended to 64-bit double.

